Demographics of M Dwarf Binary Exoplanet Hosts Discovered by TESS

M dwarfs have become increasingly important in the detection of exoplanets and the study of Earth-sized planets and their habitability. However, 20-30% of M dwarfs have companions that can impact the formation and evolution of planetary systems. We use high-resolution imaging and Gaia astrometry to detect stellar companions around M dwarf exoplanet hosts discovered by TESS and determine the projected separation and estimated stellar masses for each system. We find 47 companions around 216 M dwarfs and a multiplicity rate of $19.4\pm2.7$% that is consistent with field M dwarfs. The binary projected separation distribution is shifted to larger separations, confirming the lack of close binaries hosting transiting exoplanets seen in previous studies. We correct the radii of planets with nearby companions and examine the properties of planets in M dwarf multi-star systems. We also note three multi-planet systems that occur in close binaries ($\lesssim 50$ au) where planet formation is expected to be suppressed.

==> Table1_Initial_Observations.tex <==
\startlongtable
\movetabledown=10mm
%\begin{longrotatetable}
\begin{deluxetable*}{lcccccc}
\tabletypesize{\footnotesize}
\tablewidth{0pt}
%\tablenum{6}
%\tablecaption{Initial Table of Companion Observations\label{tab:initial_obs}}
\tablecaption{Companions observed with high-resolution imaging}
\tablehead{
\colhead{TOI} & \colhead{Instrument} & \colhead{Filter} & \colhead{Separation ($''$)} & \colhead{Position Angle ($\degr$)} & \colhead{$\Delta$ Magnitude} & \colhead{Date}} 
\startdata 
  % 212 &                                          HRCam  &                             I, I  &   0.2538, 0.255 &   358.4, 358,  &             0.7, 0.5  &                            2019-12-12, 2019-11-09  \\
  % &                                          Zorro  &                             832  &    0.23  &   184.8  &            1.05  &                            2022-07-29  \\
  % 212 &                                          HRCam  &                             I, I  &   0.9585, 0.9597  &   292.1, 291.8  &             1, 1.2  &                            2019-11-09, 2019-12-12  \\
  % &                                          Zorro  &                             832, 832  &   0.924, 0.884  &   292.4, 277.9  &             1.68 2.92  &                            2022-07-29,2022-07-29  \\
  % 224 &                                   HRCam  &                   I  &              0.0607  &         31.1  &                 0.8  &                            2019-07-14  \\
  %    &                                    Zorro  &                   562, 832  &               0.1, 0.099  &          224.8, 226.6  &                 2.07, 1  &                             2020-11-26, 2020-11-26  \\
  256\tablenotemark{b} &                                          PHARO  &                       Br-$\gamma$ &                           16.52  &                        336  &                       4.8987  &                                        2018-12-22  \\
%  454 &                                          HRCam  &                             I  &                          3.8682  &                      256.7  &                          2.2  &                                        2019-03-17  \\
  455\tablenotemark{a} &                                          HRCam  &                             I  &                          7  &                      314  &                          0.39  &                                        2019-08-12  \\
  455\tablenotemark{a} &                                          HRCam  &                             I  &                          8  &                      314  &                       1.05     &                                        2019-08-12  \\
  457 &                                'Alopeke  &                          832  &             1.039  &          222.9  &             0.67 &                2019-10-14  \\
   &                                Zorro  &                          832  &             1.056  &           44.8 &            1.06  &                2020-01-09  \\
   &                                Zorro  &                          832  &             1.059  &           44.7  &            0.71  &                2020-01-14  \\
  % 482\tablenotemark{b} &                         NESSI  &                 832  &                           0.398  &                    267.339 &                         2.43  &                 2019-10-11 \\
  %  &                         'Alopeke  &                 832  &                           0.388  &                    261.6   &                         2.9  &                2022-02-11  \\
  % 531\tablenotemark{b} &                                'Alopeke  &             832  &             0.603  &          299.533  &            2.17  &                            2022-02-16  \\
  % 543\tablenotemark{b} &                                'Alopeke  &             832  &             0.186  &          151.9  &            4.6  &                            2022-02-11  \\
  % 573 &                                NIRC2  &             Br-$\gamma$  &             1.716  &          124  &            0.9162  &                            2019-05-12  \\
  % &                             'Alopeke  &             562, 832  &             1.419, 1.519  &          227.6, 234.3  &            1.3, 1.25  &                            2020-02-15, 2020-02-15  \\
  654\tablenotemark{b} &                                          PHARO  &                Br-$\gamma$ &                     9.65 &                   120 &               4.2842  &                                        2019-06-13  \\
                       &                                          PHARO  &                Hcont  &                     9.178  &                   115  &               4.1679  &                                        2019-06-13  \\
  737 &                                NIRC2  &           Br-$\gamma$ &             0.842 &                   46  &          2.615 &                            2019-06-10  \\
  &                                NIRC2  &           Jcont  &             0.845  &                   46  &          2.6418  &                            2019-06-10  \\
  &                                'Alopeke  &            832  &             0.798  &                   47.7  &          3.25  &                             2020-02-16  \\
  % 749 &                                          NIRC2  &                  Kp, J, H  &             1.324, 1.321, 1.322  &                         70, 70, 70  &       1.9281, 1.9364, 1.9345  &                                        2019-06-25, 2019-06-25, 2019-06-25  \\
  864 &                                          Zorro  &                  562  &            0.04 &                       51.3 &       0.35  &                                        2022-01-13  \\
      &                                          Zorro  &                  832  &            0.044  &                     45.8  &      1.92  &                                        2022-01-13  \\
 1215 &                                          HRCam  &                             I  &                          1.7263  &                       84.7  &                          0.1  &                                        2019-12-14  \\
 % 1256\tablenotemark{b} &                                PHARO  &         Br-$\gamma$, Hcont  &                           1.872, 1.872  &                        140, 140  &                3.493, 3.621  &                            2021-11-11, 2021-11-11  \\
 1450 &                                          PHARO  &                Br-$\gamma$  &                    3.253  &               324.5  &                 2.936  &                                        2021-09-20  \\
      &                                          PHARO  &                Hcont  &                     3.248  &               324.7  &                 3.111  &                                        2021-09-20  \\
 1452 &                                          NIRC2  &                K  &                    3.134  &               0.36 &                 0.284  &                              2020-05-28  \\
 1634 &                                          PHARO  &                Br-$\gamma$  &                    2.538 &                      270.7  &                 2.619 &                                        2021-09-19  \\
      &                                          PHARO  &               Hcont  &                    2.535  &                      270.7  &                 2.713  &                                        2021-09-19 \\
 % 1639\tablenotemark{b} &    'Alopeke  &    832  &                           1.267  &                      351.5  &                         5.02  &    2021-10-22 \\
 1745\tablenotemark{b} &                                          PHARO  &                Br-$\gamma$   &                     0.98  &                     7.5  &   3.752  &                            2021-08-24  \\
                       &                                          PHARO  &                 Hcont  &                     0.98  &                     7.5  &   3.716  &                             2021-08-24  \\
                       &                                          PHARO  &                Br-$\gamma$  &                      1.003  &                      10  &   3.673  &                            2021-11-11  \\
                       &                                          PHARO  &                 Hcont  &                     1.003  &                   10  &  3.479  &                           2021-11-11  \\
 1746 &                                          PHARO  &                Br-$\gamma$  &                    0.943  &               173.8  &                 0.098  &                                        2021-11-11 \\
      &                                          PHARO  &                Hcont  &                    0.933  &                173.5  &               0.101  &                                        2021-11-11  \\
 1883 &                                          PHARO  &                       Br-$\gamma$  &                           15.66  &                      196.5  &                       0.9727  &                                        2021-02-24  \\
 1899\tablenotemark{b} &                                          PHARO  &                Br-$\gamma$  &                     2.31 &               355.4  &                  5.85&                                        2021-09-20  \\
                       &                                          PHARO  &                Hcont  &                     2.301  &               355.1  &                  5.885  &                                        2021-09-20  \\
 2221\tablenotemark{a} &                                          HRCam  &                             I  &                          4680.5 &                      212  &                          1.74  &                                        2020-12-03  \\
 2221\tablenotemark{a} &                                          HRCam  &                             I  &                          4682.2  &                      211.9  &                          2.72  &                                        2020-12-03  \\
 2267 &                            Speckle Polarimeter  &                             I  &                           0.408  &                     285.16  &                          1.8  &                                        2020-10-25  \\
  &                            'Alopeke  &                             832  &                           0.384  &                     279.7  &                          1.55  &                                       2021-12-09  \\
 % 2451\tablenotemark{b} &                              'Alopeke  &             832  &            0.209  &         291.617   &               3.81  &                            2022-02-12  \\
 2384   &                                          Zorro  &                             832  &   0.822  &   349.3 &       3.32       &                  2022-11-10         \\
 2455 &                              HRCam  &             I  &            0.5146  &          119.2  &               3.0  &                            2021-03-01  \\
  &                                   PHARO  &              Br-$\gamma$  &            0.505  &           120 &               4.03  &                             2021-09-19 \\
  &                                   PHARO  &              Hcont  &            0.506  &           120.2  &               2.388  &                             2021-09-19 \\
  &                                   NESSI  &              832  &            0.504  &           118.87  &               2.92  &                             2021-10-29  \\
  &                                   'Alopeke  &              832  &            0.497  &           123.9  &               4.34  &                             2021-10-16  \\
  &                                   'Alopeke  &              832 &            0.525  &           121.3  &                4.22  &                             2022-02-12  \\
 2781 &                                          HRCam  &                             I  &                          0.4471  &                       94.8  &                          1.9  &                                        2021-10-03  \\
 % 3029\tablenotemark{b} %&                                          HRCam  &                             I  &                          3.4601  &                       116.9  &                          5.9  &                                        2022-03-21  \\
 % &                                          Zorro  &                             832  &                          0.072  &                       46.7  &                          3.31  &                                        2022-05-23  \\
 3494 &                                          HRCam  &                             I &                          0.5927  &                      293.1  &                          2.9  &                                        2021-07-15  \\
      &                                          HRCam  &                             I  &                         0.6017  &                      293.1  &                          2.9  &                                        2022-06-13  \\
      &                                          Zorro  &                             832  &                         0.605  &                     293.1  &                          3.02  &                                        2023-04-07  \\
 % 3528\tablenotemark{b} &                                          PHARO  &                Br-$\gamma$, Hcont  &                            1.57, 1.57  &                      180.5, 180.5  &                 0.197, 0.187  &                                        2021-08-08, 2021-08-08  \\
 % 3583\tablenotemark{b} &                                          NIRC2  &                             K  &                           0.589  &                      156.3  &                        4.054  &                                        2021-08-28  \\
 % 4261\tablenotemark{b} &                                   Zorro  &                          832  &                   0.128  &                234.7  &                    6.06  &                            2022-03-21  \\
 4325\tablenotemark{b} &                                          HRCam  &                             I  &                   3.2583  &                233.5  &                      3.7  &                                        2021-10-18  \\
 4325\tablenotemark{b} &                                          HRCam  &                             I  &                  9.2699  &               214.6  &                     2.5 &                                        2021-10-18  \\
 4349 &                                 NIRC2    &                          K  &                  2.681   &               347.1   &                    2.45  &                            2021-08-28  \\
 &                                  HRCam   &                           I  &                  2.7053    &              12.4   &                     2.9  &                             2021-10-01  \\
 4446\tablenotemark{c} &                                   NIRC2  &                          K  &                  2.725   &                7.6   &                   6.72  &                            2012-06-24  \\
 4446\tablenotemark{c} &                                   NIRC2  &                          K  &                  3.298    &                68.4    &                   6.151   &                            2012-06-24  \\
 4889 &                                   Zorro  &                          562  &                  0.119   &                226.2    &                   3.12   &                            2022-03-21  \\
      &                                   Zorro  &                          832  &                  0.118    &               222.9    &                   0.67   &                            2022-03-21  \\
 &                                   HRCam  &                          I  &                 0.1268    &                47.5    &                   0.0   &                            2022-06-11  \\
 % 5031\tablenotemark{b} &                                   Zorro  &                          562, 832  &                   0.648, 0.655  &                227.3, 226.6   &                    2.35, 2.2  &                            2022-03-19, 2022-03-19  \\
\enddata
\tablenotetext{a}{Companion parameters on ExoFOP refer to the outer components of a triple system. Here we show the companion parameters with respect to the primary star. See Section~\ref{hrcomps} for details.}%The separation and position angle reported here are inferred from the WDS, while the delta magnitudes are calculated from \citet{2019AJ....158..152W}. See text for details.}
\tablenotetext{b}{Unbound, see Section \ref{boundcomps}}
\tablenotetext{c}{KOI-245, observed by Kraus et al.~2016, ExoFOP observations extracted from Furlan et al.~2017.}
\end{deluxetable*}
%\end{longrotatetable}

==> Table2_Gaia_Companions_Refined.tex <==
\startlongtable
\movetabledown=10mm
\begin{deluxetable*}{lhcccccccc}
\tabletypesize{\scriptsize}
\tablewidth{0pt} 
\tablecaption{Companions detected using proper motions and parallaxes \label{tab:gaiacomps}}
\tablehead{
\colhead{TOI} & \nocolhead{TIC} & \colhead{Sep. ($''$)} & \colhead{Pos. Angle ($\degr$)} & \colhead{$\Delta$ Mag. (Gaia)} & \colhead{Mag. (Gaia)} & \colhead{Parallax (mas)} & \colhead{PM RA (mas)} & \colhead{PM Dec (mas)} & \colhead{Add.~Ref}}
\startdata 
218 &   32090583 &    13.53 & 226.09 &              0.15 &   14.63 &    19.03$\pm$0.02 &   139.03$\pm$0.02 &   191.18$\pm$0.02 &  M20,E21 \\
 &   32090583 &     &         &        &   14.79 &    19.03$\pm$0.02 &  139.90$\pm$0.02  &  191.23$\pm$0.02  &  \\
277\tablenotemark{a} &  439456714 &    17.25 & 352.37 &               0.30 &   12.78 &    15.41$\pm$0.02 &  -115.33$\pm$0.02 &  -249.42$\pm$0.01 &  M20,E21 \\
 &  439456714 &     &          &       &   12.47 &    15.44$\pm$0.02 &  -113.72$\pm$0.01 & -248.93$\pm$0.02  &   \\
457\tablenotemark{b} &   89256802 &     1.03 & 222.01 &               0.42 &   15.63 &     7.98$\pm$0.07 &    83.50$\pm$0.03 &    47.84$\pm$0.05 &  M20,E21 \\
 &   89256802 &      &       &          &   16.05 &     7.95$\pm$0.09 &   78.78$\pm$0.07  &   51.77$\pm$0.05  &   \\
468\tablenotemark{a} &   33521996 &   329.51 & 256.01 &               7.67 &   14.34 &     5.89$\pm$0.02 &    -2.57$\pm$0.01 &     7.37$\pm$0.05 &          \\
 &   33521996 &    &         &        &   5.91 &  6.68$\pm$0.02    &   -2.49$\pm$0.01  &   7.47$\pm$0.01   &          \\
488 &  452866790 &    49.26 & 222.79 &               3.47 &   12.45 &    36.61$\pm$0.02 &  -403.20$\pm$0.02 &  -380.93$\pm$0.01 &  M20,E21 \\
 &  452866790 &     &       &          &   15.92 &    36.45$\pm$0.07 & -399.42$\pm$0.04  &  -380.74$\pm$0.05 &   \\
507 &  348538431 &    73.46 & 340.15 &               0.47 &   14.48 &     9.10$\pm$0.02 &    47.71$\pm$0.01 &   -15.27$\pm$0.01 &  M20,E21 \\
 &  348538431 &     &        &         &   14.95 &     9.12$\pm$0.02 &  47.69$\pm$0.01   &  -15.04$\pm$0.02  &   \\
756 &   73649615 &    11.09 & 163.20 &               1.34 &   13.68 &    11.61$\pm$0.02 &  -216.50$\pm$0.01 &    29.20$\pm$0.01 &  M20,E21 \\
 &   73649615 &     &         &        &   15.02 &    11.61$\pm$0.03 & -215.7$\pm$0.02  &  29.5$\pm$0.02   &   \\
762 &  178709444 &     3.20 & 239.54 &               3.29 &   14.93 &    10.12$\pm$0.02 &  -159.17$\pm$0.02 &   -24.78$\pm$0.02 &  M20,E21 \\
 &  178709444 &      &         &        &   18.22 &    9.79$\pm$0.14 &  -157.37$\pm$0.1 &  -24.38$\pm$0.1  &   \\
1215\tablenotemark{b} &  453260209 &     1.76 & 84.55 &               0.12 &   11.42 &    28.89$\pm$0.02 &  -131.35$\pm$0.02 &  -117.48$\pm$0.02 &  M20,E21 \\
 &  453260209 &      &        &         &   11.42 &    28.89$\pm$0.02 & -143.02$\pm$0.02  & -120.86$\pm$0.02  &   \\
1227\tablenotemark{a} &  360156606 &   511.83 & 270.53 &               3.26 &   15.22 &     9.90$\pm$0.02 &   -40.29$\pm$0.02 &   -10.81$\pm$0.02 &          \\
 &  360156606 &    &         &        &  11.96  &     8.54$\pm$0.65 & -42.09$\pm$0.54   & -8.72$\pm$0.55   &          \\
1450\tablenotemark{b} &  377293776 &     3.39 & 323.67 &              3.78 &   11.24 &    44.56$\pm$0.02 &    69.99$\pm$0.02 &    11.24$\pm$0.01 &  M20,E21 \\
 &  377293776 &      &       &          &   15.02 &    44.52$\pm$0.03 &  83.31$\pm$0.03   & 143.77$\pm$0.03    &   \\
1452\tablenotemark{b} &  420112589 &     3.18 & 0.03 &               0.23 &   13.60 &    32.78$\pm$0.01 &     7.80$\pm$0.01 &   -74.08$\pm$0.01 &  M20,E21 \\
 &  420112589 &      &       &          &   13.83 &    32.79$\pm$0.01 &   6.85$\pm$0.01   &  -82.22$\pm$0.01  &   \\
1634\tablenotemark{b} &  201186294 &     2.54 & 269.36 &               3.40 &   12.19 &    28.51$\pm$0.02 &    81.35$\pm$0.01 &    13.55$\pm$0.01 &  M20,E21 \\
 &  201186294 &      &        &         &   15.59 &    28.62$\pm$0.11 &  80.64$\pm$0.07   &   14.54$\pm$0.09  &   \\
1696 &  470381900 &   426.19 & 208.66 &               4.80 &   15.31 &    15.48$\pm$0.03 &    12.87$\pm$0.03 &   -19.05$\pm$0.02 &          \\
 &  470381900 &    &           &      &   15.31 &    9.89$\pm$1.94 &  13.99$\pm$0.89   &  -26.81$\pm$1.49  &          \\
1746\tablenotemark{b} &  232650365 &     0.93 & 171.41 &               0.15 &   13.80 &    22.69$\pm$0.11 &     7.40$\pm$0.13 &    55.38$\pm$0.11 &  M20,E21 \\
 &  232650365 &      &        &         &   13.80 &    22.64$\pm$0.04 &   9.37$\pm$0.04   &   53.82$\pm$0.06  &   \\
1763 &  441739871 &    15.11 & 66.61 &               0.71 &   13.94 &    11.35$\pm$0.01 &    -5.01$\pm$0.01 &   -38.44$\pm$0.01 &  M20,E21 \\
 &  441739871 &     &         &        &   14.65 &    11.34$\pm$0.02 &  -4.41$\pm$0.02   & -38.18$\pm$0.02   &   \\
1801 &  119584412 &   105.05 & 21.97 &              2.36 &   10.83 &    32.37$\pm$0.02 &  -204.89$\pm$0.02 &    41.84$\pm$0.02 &  M22,E21 \\
 &  119584412 &    &          &       &   13.19 &    32.37$\pm$0.02 &  -204.91$\pm$0.02 &   42.49$\pm$0.01  &   \\
1883\tablenotemark{b} &  348755728 &    15.75 & 194.94 &              0.69 &   14.50 &     8.51$\pm$0.02 &    30.78$\pm$0.02 &     2.84$\pm$0.02 &  M20,E21 \\
 &  348755728 &       &        &         &  15.19  &    8.58$\pm$0.04  &   30.58$\pm$0.03  &   3.15$\pm$0.03   &   \\
1883 &  348755728 &   261.14 & 236.20 &               6.02 &   14.50 &     8.51$\pm$0.02 &    30.78$\pm$0.02 &     2.84$\pm$0.02 &          \\
 &  348755728 &    &         &        &   20.52 &     13.12$\pm$2.56 &  18.84$\pm$1.70   &  7.04$\pm$1.40    &          \\%parallax/error>5? - code looks at combined main and companion parallax/error
2068 &  417931300 &    19.99 & 65.49 &               0.23 &   12.21 &    18.87$\pm$0.01 &  -197.94$\pm$0.01 &    -6.06$\pm$0.01 &  M21,E21 \\
 &  417931300 &     &        &         &   12.44 &    18.86$\pm$0.01 & -200.44$\pm$0.01  &  -7.29$\pm$0.01   &   \\
2072 &  900715901 &     2.99 & 130.52 &               0.92 &   12.70 &    25.63$\pm$0.02 &  -184.97$\pm$0.02 &   -87.24$\pm$0.02 &  M21,E21 \\
 &  900715901 &      &       &          &   13.61 &    25.55$\pm$0.02 & -184.59$\pm$0.02  & -92.03$\pm$0.01   &   \\
2084 &  441738827 &    12.25 & 191.19 &               6.29 &   14.39 &     8.75$\pm$0.02 &    47.73$\pm$0.02 &    36.76$\pm$0.01 &  M21,E21 \\
 &  441738827 &     &        &         &   14.65 &     8.79$\pm$0.75 &  49.1$\pm$0.56   &  38.89$\pm$0.67   &   \\
2094 &  356016119 &    10.71 & 215.71 &               4.60 &   13.43 &    19.91$\pm$0.01 &   -55.30$\pm$0.01 &    -0.13$\pm$0.01 &  M21,E21 \\
 &  356016119 &     &        &         &   18.03 &    20.06$\pm$0.12 & -54.38$\pm$0.11   &  1.27$\pm$0.12   &   \\
2205 &  260298958 &     2.15 & 83.39 &               3.19 &   16.13 &     2.41$\pm$0.03 &    -2.33$\pm$0.03 &    27.63$\pm$0.03 &      M21 \\ %corrected PA!?
 &  260298958 &      &       &          &   19.32 &     2.39$\pm$0.14 &  -2.12$\pm$0.15   &  27.47$\pm$0.13   &      \\
2205 &  260298958 &    21.83 & 255.41 &               2.66 &   16.13 &     2.41$\pm$0.03 &    -2.33$\pm$0.03 &    27.63$\pm$0.03 &      M21 \\
 &  260298958 &     &         &        &   18.79 &     2.39$\pm$0.14 &  -2.12$\pm$0.13   &   27.47$\pm$0.15  &       \\
2293 &   71347873 &     4.66 & 1.24 &               4.07 &   12.86 &    15.94$\pm$0.02 &    45.22$\pm$0.01 &  -120.70$\pm$0.01 &  M21,E21 \\
 &   71347873 &      &        &         &   16.93 &    16.08$\pm$0.06 &  45.11$\pm$0.05   &  -123.74$\pm$0.04 &   \\
2384\tablenotemark{b} &  382602147 &     0.84 & 350.29 &               3.16 &   14.39 &     5.32$\pm$0.04 &     9.26$\pm$0.04 &   -52.66$\pm$0.04 &  M21,E21 \\
 &  382602147 &      &        &         &   17.55 &     5.05$\pm$0.17 &   8.01$\pm$0.19   &  -51.04$\pm$0.44  &   \\
3397 &  154616309 &   536.57 & 268.28 &               6.30 &   14.29 &     5.50$\pm$0.02 &    14.50$\pm$0.01 &     9.73$\pm$0.01 &          \\
 &  154616309 &    &          &       &   20.59 &     12.09$\pm$2.24 &  3.48$\pm$1.77   &  10.89$\pm$1.1    &          \\%parallax/error > 5?
3714 &  155867025 &     2.67 & 106.42 &               4.56 &   14.29 &     8.84$\pm$0.02 &    19.83$\pm$0.02 &   -70.76$\pm$0.01 &  M23,E21 \\
 &  155867025 &      &        &         &   18.85 &     8.85$\pm$0.23 &  18.8$\pm$0.11   &  -70.67$\pm$0.2   &   \\
3984 &   20182780 &     3.27 & 343.08 &               4.43 &   14.65 &     9.18$\pm$0.02 &   -48.95$\pm$0.01 &    42.65$\pm$0.02 &  M23,E21 \\
 &   20182780 &      &         &        &   19.08 &     9.06$\pm$0.2 &  -50.38$\pm$0.16  &  40.95$\pm$0.13   &   \\
4325 &  202185707 &    25.30 & 356.26 &               2.46 &   12.98 &    19.53$\pm$0.02 &    74.70$\pm$0.02 &  -169.87$\pm$0.02 &  M23,E21 \\
 &  202185707 &     &          &       &   15.44 &    19.51$\pm$0.04 &  74.78$\pm$0.03   & -170.67$\pm$0.03  &   \\
4336 &  166184428 &     6.30 & 302.79 &               0.19 &   12.25 &    44.53$\pm$0.04 &   151.81$\pm$0.03 &    68.40$\pm$0.02 &          \\
 &  166184428 &      &        &         &   12.43 &    44.55$\pm$0.04 &  150.41$\pm$0.03  &  71.66$\pm$0.03   &          \\
4336 &  166184428 &    98.50 & 197.59 &               1.01 &   12.25 &    44.53$\pm$0.04 &   151.81$\pm$0.03 &    68.40$\pm$0.02 &          \\
 &  166184428 &     &         &        &   13.26 &    44.50$\pm$0.02 &  151.99$\pm$0.01  &   71.80$\pm$0.01  &          \\
4349\tablenotemark{b} &  313889049 & 2.68 & 12.35 &                3.04 &   12.66 &    13.89$\pm$0.02 &   278.22$\pm$0.02 &   105.50$\pm$0.02 &  M23,E21 \\
 &  313889049 &      &       &          &   15.70 &    13.86$\pm$0.11 &  280.63$\pm$0.08  &  108.14$\pm$0.09  &   \\
4642\tablenotemark{a} &  336961891 &   110.77 & 238.42 &               0.54 &   13.27 &    42.44$\pm$0.02 &    92.00$\pm$0.02 &  -122.04$\pm$0.02 &      E21 \\
 &  336961891 &    &         &        &   12.73 &    42.53$\pm$0.03 &  94.02$\pm$0.02   & -120.39$\pm$0.03  &       \\
4668 &  142938659 &    20.91 & 194.95 &               0.02 &   15.16 &     9.43$\pm$0.02 &    35.72$\pm$0.02 &    -4.42$\pm$0.02 &          \\
 &  142938659 &     &        &         &   15.19 &     9.42$\pm$0.03 &  35.24$\pm$0.02   &  -4.31$\pm$0.02   &          \\
4858 &  262499797 &    36.34 & 35.89 &               4.06 &   16.05 &     5.04$\pm$0.03 &    54.19$\pm$0.03 &   -92.53$\pm$0.03 &      E21 \\
 &  262499797 &     &         &        &   20.11 &     4.41$\pm$0.51 &  51.91$\pm$0.52   & -93.23$\pm$0.49   &       \\
4991 &  247180220 &    30.01 & 150.17 &                3.08 &   15.75 &     2.91$\pm$0.04 &    10.80$\pm$0.03 &    -3.03$\pm$0.02 &      E21 \\
 &  247180220 &     &          &       &   18.83 &     2.29$\pm$0.23 &  10.09$\pm$0.14  &  -3.01$\pm$0.2   &       \\
\enddata
\tablenotetext{a}{Detected companion is brighter than the TOI. For these systems, the mass ratio is calculated using the brighter star as primary.}
\tablenotetext{b}{Companion also detected with high-resolution imaging.}
\tablecomments{References for previously identified CPM companions: M20 - \citet{2020AN....341..996M}, M21 - \citet{2021AN....342..840M}, M22 - \citet{2022AN....34324017M}, M23 - \citet{2023AN....34430055M}, E21 - \citet{2021MNRAS.506.2269E}}
\end{deluxetable*}


==> Table3_Final_Companions_Refined.tex <==
\startlongtable
\begin{longrotatetable}
\begin{deluxetable*}{lcccccccCC}
\tabletypesize{\footnotesize}
\tablewidth{0pt}
\tablecaption{Observed and derived properties of analyzed companions\label{tab:final_comp}}
\tablehead{
\colhead{TOI} & \colhead{Separation ($''$)} & \colhead{Pri.~Mag (filter)} & \colhead{Sec.~Mag (Calc.)} & \colhead{T$_{\mathrm{eff}}$ (K)} & \colhead{Distance (pc)} & \colhead{Proj.~Sep (AU)} & \colhead{$M_{\mathrm{pri}}$ ($M_{\odot}$)} & \colhead{$M_{\mathrm{comp}}$ ($M_{\odot}$)} & \colhead{RUWE}} 
\startdata 
  218 &            13.53 &       14.63 (G) &         14.79 &                3146 &        52.56 &             710.96 &  0.18 & 0.18 &   1.12 \\
  277\tablenotemark{a} &            17.25 &       12.47 (G) &         12.78 &                3748 &        64.91 &            1119.47 &  0.57 & 0.54 &   1.28 \\
  455 &             7.00 &        8.04 (I) &          8.43 &                3562 &         6.86 &              48.05 &  0.44 & 0.4 &   1.07 \\
  455 &             8.00 &        8.04 (I) &          9.09 &                3562 &         6.86 &              54.91 &  0.44 & 0.27 &   1.07 \\
  457 &             1.06 &       10.87 (I) &         11.93 &                3054 &       125.36 &             130.38 &  0.16 & 0.12 &   1.03 \\
  488 &            49.26 &       12.45 (G) &         15.92 &                3332 &        27.31 &            1345.51 &  0.27 & 0.09 &   1.30 \\
  507 &            73.46 &       14.48 (G) &         14.95 &                3338 &       109.94 &            8076.36 &  0.27 & 0.23 &   1.10 \\
  737 &             0.84 &        6.55 (K) &          9.17 &                3394 &       291.99 &             245.86 &  0.37 & 0.10 &   1.01 \\
  756 &            11.09 &       13.68 (G) &         15.02 &                3614 &        86.13 &             955.37 &  0.47 & 0.37 &   1.24 \\
  762 &             3.20 &       14.93 (G) &         18.22 &                3399 &        98.84 &             315.99 &  0.37 & 0.12 &   1.03 \\
  864 &             0.04 &        8.30 (I) &         10.22 &                3460 &        38.01 &               1.67 &  0.40 & 0.18 &   1.18 \\
 1215 &             1.73 &        7.31 (I) &          7.41 &                3751 &        34.62 &              59.76 &  0.54 & 0.54 &   1.31 \\
 1227\tablenotemark{a} &           511.83 &       11.96 (G) &         15.22 &                3050 &       100.96 &           51675.47 &  0.44 & 0.16 &   1.06 \\
 1450 &             3.25 &        6.55 (K) &          9.49 &                3407 &        22.44 &              73.01 &  0.37 & 0.09 &   1.01 \\
 1452 &             3.13 &        7.10 (K) &          7.38 &                3248 &        30.50 &              95.60 &  0.27 & 0.23 &   1.41 \\
 1634 &             2.54 &        6.18 (K) &          8.80 &                3455 &        35.07 &              89.01 &  0.40 & 0.12 &   1.23 \\
 1696 &           426.19 &       15.31 (G) &         20.11 &                3181 &        64.62 &           27540.46 &  0.23 & 0.08 &   1.12 \\
 1746 &             0.94 &        7.10 (K) &          7.20 &                3340 &        44.08 &              41.57 &  0.27 & 0.27 &   4.45 \\
 1763 &            15.11 &       13.94 (G) &         14.65 &                3520 &        88.14 &            1331.82 &  0.44 & 0.37 &   1.26 \\
 1801 &           105.05 &       10.83 (G) &         13.19 &                3815 &        30.89 &            3245.32 &  0.57 & 0.27 &   1.04 \\
 1883 &            15.66 &        11.53 (K) &        12.50 &                3477 &       117.53 &            1840.60 &  0.40 & 0.27 &   1.12 \\
 1883 &            261.14 &        14.50 (G) &          20.52 &                3477 &       117.53 &         30693.06 &       0.4 & 0.08 & 1.12 \\
 2068 &            19.99 &       12.21 (G) &         12.44 &                3700 &        53.00 &            1059.22 &  0.50 & 0.47 &   1.16 \\
 2072 &             2.99 &       12.70 (G) &         13.61 &                3546 &        39.02 &             116.62 &  0.44 & 0.37 &   1.54 \\
 2084 &            12.25 &       14.39 (G) &         20.68 &                3630 &       114.29 &            1399.48 &  0.47 & 0.09 &   1.06 \\
 2094 &            10.71 &       13.43 (G) &         18.03 &                3457 &        50.22 &             538.08 &  0.40 & 0.10 &   1.32 \\
 2205 &            2.15 &       16.13 (G) &         19.32 &                3653 &       414.95 &            892.04 &     0.50 & 0.184 & 1.05 \\
 2205 &            21.83 &       16.13 (G) &         18.79 &                3653 &       414.95 &            9059.55 &  0.50 & 0.23 &   1.05 \\
 2221 &             4680.50 &        8.04 (G) &          9.78 &                3588 &         9.71 &              45466.82 &  0.44 & 0.23 &   0.93 \\
 2221 &             4682.20 &        8.04 (G) &         10.76 &                3588 &         9.71 &              45483.34 &  0.44 & 0.16 &   0.93 \\
 2267 &             0.38 &       10.87 (I) &         12.42 &                3022 &        22.55 &               8.66 &  0.16 & 0.10 &  13.71 \\
 2293 &             4.66 &       12.86 (G) &         16.93 &                3668 &        62.75 &             292.63 &  0.50 & 0.16 &   1.23 \\
 2384 &             0.82 &      7.63 (I) &         10.96 &              3678 &       187.90 &             154.46 &  0.5 & 0.16 &   3.21 \\
 2455 &             0.51 &        5.98 (K) &         10.01 &                3553 &       100.98 &              50.99 &  0.44 & 0.09 &   7.79 \\
 2781 &             0.45 &        7.03 (I) &          8.93 &                3868 &       161.21 &              72.08 &  0.57 & 0.37 &   9.34 \\
 3397 &           536.57 &       14.29 (G) &         20.59 &                3811 &       181.78 &           97537.93 &  0.57 & 0.09 &   0.99 \\
 3494 &             0.59 &        9.78 (I) &         12.68 &                3230 &        34.07 &              20.19 &  0.23 & 0.09 &   3.72 \\
 3714 &             2.67 &       14.29 (G) &         18.85 &                3538 &       113.14 &             302.05 &  0.44 & 0.10 &   1.15 \\
 3984 &             3.27 &       14.65 (G) &         19.08 &                3422 &       108.88 &             356.11 &  0.37 & 0.09 &   1.10 \\
 4325 &            25.30 &       12.98 (G) &         15.44 &                3896 &        51.21 &            1295.73 &  0.57 & 0.27 &   1.18 \\
 4336 &             6.30 &       12.25 (G) &         12.43 &                3365 &        22.45 &             141.47 &  0.37 & 0.37 &   1.86 \\
 4336 &             98.50 &       12.25 (G) &         13.26 &                3365 &        22.45 &             2211.68 &  0.37 & 0.23 &   1.86 \\
 4349 &             2.68 &        5.15 (K) &          7.60 &                3851 &        71.99 &             193.01 &  0.57 & 0.23 &   1.57 \\
 4642\tablenotemark{a} &           110.77 &       12.73 (G) &         13.27 &                3266 &        23.56 &            2609.66 &  0.37 & 0.27 &   1.35 \\
 4668 &            20.91 &       15.16 (G) &         15.19 &                3210 &       106.00 &            2216.60 &  0.23 & 0.23 &   1.06 \\
 4858 &            36.34 &       16.05 (G) &         20.11 &                3333 &       198.49 &            7212.79 &  0.27 & 0.09 &   1.03 \\
 4991 &           165.15 &       15.75 (G) &         20.47 &                3601 &       343.08 &           56658.57 &  0.47 & 0.18 &   1.04 \\
\enddata
\tablenotetext{a}{The TOI is fainter than the detected companion and assumed to be the secondary.}
\tablecomments{Parenthetical notes in the primary magnitude column indicate what band the data are in. I = I Band, K = K Band, G = Gaia Band}
\end{deluxetable*}
\end{longrotatetable}

==> Table4_Radius_Corrections.tex <==
\startlongtable
\movetabledown=10mm
%\begin{longrotatetable}
\begin{deluxetable*}{lccc}
\tabletypesize{\footnotesize}
\tablewidth{0pt}
%\tablenum{6}
\tablecaption{Corrected planetary radii for TOIs with previously unresolved companions\label{tab:radii_cor}}
\tablehead{
\colhead{TOI} & \colhead{Uncorrected Radius ($R_{\earth}$)} & \colhead{Correction Factor} & \colhead{Corrected Radius ($R_{\earth}$)}} 
\startdata 
%  224.01 &                          17.18 &             1.182 &                       20.313 \\
%  573.01 &                         19.854 &             1.196 &                       23.743 \\
%  749.01 &                         14.372 &             1.081 &                       15.542 \\
  864.01 &                          1.005 &             1.082 &                        1.087 \\
 1215.01 &                          0.879 &             1.383 &                        1.216 \\
 2267.01 &                          1.273 &             1.114 &                        1.418 \\
 2267.02 &                          0.901 &             1.114 &                        1.003 \\
 2267.03 &                          0.913 &             1.114 &                        1.017 \\
 2455.01 &                         14.327 &             1.012 &                       14.501 \\
 2781.01 &                          5.942 &             1.083 &                        6.438 \\
 3494.01 &                          2.217 &             1.034 &                        2.292 \\
\enddata
\end{deluxetable*}

==> Table5_FP_companions.tex <==
\startlongtable
\movetabledown=10mm
%\begin{longrotatetable}
\begin{deluxetable*}{lcccccc}
\tabletypesize{\footnotesize}
\tablewidth{0pt}
%\tablenum{6}
%\tablecaption{Initial Table of Companion Observations\label{tab:initial_obs}}
\tablecaption{Companions detected around FP, APC, or giant star TOIs\label{tab:initial_obs}}
\tablehead{
\colhead{TOI} & \colhead{Instrument} & \colhead{Filter} & \colhead{Separation (")} & \colhead{Position Angle ($\degr$)} & \colhead{Delta Magnitude} & \colhead{Date}} 
\startdata 
  % 212 &                                          HRCam  &                             I, I  &   0.2538, 0.255 &   358.4, 358,  &             0.7, 0.5  &                            2019-12-12, 2019-11-09  \\
  212 &                                          Zorro  &                             832  &    0.23  &   184.8  &            1.05  &                            2022-07-29  \\
  % 212 &                                          HRCam  &                             I, I  &   0.9585, 0.9597  &   292.1, 291.8  &             1, 1.2  &                            2019-11-09, 2019-12-12  \\
  212 &                                          Zorro  &                             832  &   0.924&   292.4 &             1.68  &                            2022-07-29 \\
   &                                          Zorro  &                             832  &   0.884  &   277.9  &             2.92  &                            2022-07-29  \\
  % 224 &                                   HRCam  &                   I  &              0.0607  &         31.1  &                 0.8  &                            2019-07-14  \\
   224  &                                    Zorro  &                   562  &               0.1  &          224.8  &                 2.07  &                             2020-11-26  \\
        &                                    Zorro  &                   832  &              0.099  &           226.6  &                 1.0  &                            2020-11-26  \\
   % 454 &                                          HRCam  &                             I  &                          3.8682  &                      256.7  &                          2.2  &                                        2019-03-17  \\
  482 &                         NESSI  &                 832  &                           0.398  &                    267.3 &                         2.43  &                 2019-10-11 \\
   &                         'Alopeke  &                 832  &                           0.388  &                    261.6   &                         2.9  &                2022-02-11  \\
  531 &                                'Alopeke  &             832  &             0.603  &          299.5  &            2.17  &                            2022-02-16  \\
  543 &                                'Alopeke  &             832  &             0.186  &          151.9  &            4.6  &                            2022-02-11  \\
  573 &                                NIRC2  &             Br-$\gamma$  &             1.716  &          124  &            0.9162  &                            2019-05-12  \\
  &                             'Alopeke  &             562  &             1.419  &          227.6  &            1.3  &                            2020-02-15  \\
  &                             'Alopeke  &             832  &             1.519  &          234.3  &            1.25  &                            2020-02-15  \\
  749 &                                          NIRC2  &                  Kp &             1.324 &                         70 &       1.9281 &                                        2019-06-25 \\
   &                                          NIRC2  &                  J  &             1.321  &                         70  &       1.9364  &                                        2019-06-25  \\
   &                                          NIRC2  &                   H  &             1.322  &                         70  &      1.9345  &                                        2019-06-25  \\
  1234 &                                          PHARO  &                  Kcont &             2.137 &                         122 &       1.666 &                                        2023-08-10 \\
   &                                          PHARO  &                  Hcont  &             2.374  &                         106.64  &       2.181  &                                        2023-08-10  \\
 1256 &                                PHARO  &         Br-$\gamma$  &                           1.872 &                        140 &                3.493 &                            2021-11-11 \\
     &                                PHARO  &         Hcont  &                           1.872  &                        140  &                3.621  &                             2021-11-11  \\
 1639 &    'Alopeke  &    832  &                           1.267  &                      351.5  &                         5.02  &    2021-10-22 \\
 2451 &                              'Alopeke  &             832  &            0.209  &         291.6   &               3.81  &                            2022-02-12  \\
 3029 %&                                          HRCam  &                             I  &                          3.4601  &                       116.9  &                          5.9  &                                        2022-03-21  \\
 &                                          Zorro  &                             832  &                          0.072  &                       46.7  &                          3.31  &                                        2022-05-23  \\
 3528 &                                          PHARO  &                Br-$\gamma$  &                            1.57 &                      180.5 &                 0.197 &                           2021-08-08 \\
      &                                          PHARO  &                Hcont  &                            1.57  &                      180.5  &                 0.187  &                          2021-08-08 \\
 3583 &                                          NIRC2  &                             K  &                           0.589  &                      156.3  &                        4.054  &                                        2021-08-28  \\
 4261 &                                   Zorro  &                          832  &                   0.128  &                234.7  &                    6.06  &                            2022-03-21  \\
 5031 &                                   Zorro  &                          562 &                   0.648 &                227.3  &                    2.35  &                            2022-03-19  \\
     &                                   Zorro  &                          832  &                   0.655  &                226.6   &                    2.2  &                            2022-03-19  \\
\enddata
\end{deluxetable*}
%\end{longrotatetable}
